Constant Degree Direct Product Testers with Small Soundness

Let $X$ be a $d$-dimensional simplicial complex. A function $F\colon X(k)\to \{0,1\}^k$ is said to be a direct product function if there exists a function $f\colon X(1)\to \{0,1\}$ such that $F(\sigma) = (f(\sigma_1), \ldots, f(\sigma_k))$ for each $k$-face $\sigma$. In an effort to simplify components of the PCP theorem, Goldreich and Safra introduced the problem of direct product testing, which asks whether one can test if $F\colon X(k)\to \{0,1\}^k$ is correlated with a direct product function by querying $F$ on only $2$ inputs. Dinur and Kaufman conjectured that there exist bounded degree complexes with a direct product test in the small soundness regime. We resolve their conjecture by showing that for all $\delta>0$, there exists a family of high-dimensional expanders with degree $O_{\delta}(1)$ and a $2$-query direct product tester with soundness $\delta$. We use the characterization given by a subset of the authors and independently by Dikstein and Dinur, who showed that some form of non-Abelian coboundary expansion (which they called "Unique-Games coboundary expansion") is a necessary and sufficient condition for a complex to admit such direct product testers. Our main technical contribution is a general technique for showing coboundary expansion of complexes with coefficients in a non-Abelian group. This allows us to prove that the high dimensional expanders constructed by Chapman and Lubotzky satisfies the necessary conditions, thus admitting a 2-query direct product tester with small soundness.

==> old.tex <==
%%%%%%%%%Base case of induction for Johnson %%%%%%%%
\subsection{Johnson}
Consider the Johnson graph $J = J(n,k,k-1)$, where there is an edge between two sets that have intersection $k-1$. Given an ordering $\pi:[n] \rightarrow [n]$, we fix an ordering of every vertex $U \in J$ as follows: $O(U) = [u_1,\ldots, u_k]$ such that this is the lexicographically smallest string with respect to the ordering $\{\pi(1),\ldots, \pi(n)\}$.

\begin{mdframed}
\begin{algo}[$\Phi, J$]\label{alg:propagation}\mbox{}\\
Input: UG instance $\Phi$ on $J=J(n,k,k-1)$.\\
Output: A function $L: V(J) \rightarrow \{S_m\}$.

\begin{enumerate}
\item Choose a random vertex $U_0$ and a random ordering $\pi: [n] \rightarrow [n]$. Assign $L(U_0) = \text{id}$.
\item Let $U_0 = \{u_1,\ldots, u_k\}$ with respect to $\pi$. For every vertex $V = \{v_1,\ldots, v_k\}$ (with respect to $\pi$), choose the following path from $U_0$ to $V$: 
\[U_0 \rightarrow \{v_1,u_2,\ldots, u_k\} \rightarrow \ldots \rightarrow \{v_1,\ldots,v_k\}.\]
Assign $V$ the permutation we get by propagating the label of $U_0$ along this path: 
\[L(V) = \text{id} \circ \pi_{U_0 \rightarrow \{v_1,u_2,\ldots, u_k\}} \circ \ldots \circ \pi_{\{v_1,\ldots,v_{k-1},u_k\}\rightarrow V}.\]
\end{enumerate}
\end{algo}
\end{mdframed}

We can now analyse the expected edges violated by $L$.

\begin{claim}
Every square in $J$ can be triangulated by $O(1)$ triangles.    
\end{claim}

\begin{claim}\label{claim:sq}
Let $C_{U_0,V,W}$ be the cycle $U_0 \rightarrow V \rightarrow W \rightarrow U_0$, where $U_0 \rightarrow V$ and $W \rightarrow U_0$ are the paths we chose in Algorithm~\ref{alg:propagation}. $C_{U_0,V,W}$ can be triangulated by $O(k)$ triangles.    
\end{claim}

\begin{proof}
Let $V_1,\ldots, V_k$ be the vertices along the path from $U_0 \rightarrow V$ and same for $W$. First note that there is an edge between $V_i$ and $W_i$.

Therefore we have broken the cycle $C$ into $1$ triangle and $O(k)$ squares, and using Claim~\ref{claim:sq} we can triangulate each square using $O(1)$ triangles, thus getting an $O(k)$ size triangulation for $C$.
\end{proof}

\begin{lemma}
Let $\Phi$ be an instance where at most $\eps$-fraction of triangles are inconsistent. Then in expectation over the choice of $U_0,\pi$, the algorithm above produces an assignment violating at most $O(k\eps)$-fraction of edges.    
\end{lemma}

\begin{proof}
This follows by the symmetry of all triangles.    
\end{proof}


%%%%%%Local to global for vanishing cohomology%%%%%%%%%

\subsection{Local to Global for Vanishing Cohomology}
In this section we prove that if all local restrictions of an $\eps$-product distribution have vanishing cohomology then the global distribution also has vanishing cohomology.

\mitali{remove?}

\begin{lemma}
Let $\mu$ be a distribution over the domain $X_1 \times \ldots \times X_6$. Assume that $\mu$ satisfies the following properties:
\begin{enumerate}
    \item $\mu$ is $\eps$-product.
    \item $\mu$ has local vanishing cohomology (Definition~\ref{def:local-vc}).
    \item Inductive hypothesis: For all $V \in \supp(\mu|_{\{1\}})$, the tripartite graph $T(\{2\},\{3,4\},\{5,6\};\mu|(X_1 = V)$, has vanishing cohomology. Same holds for coordinates $3$ and $5$.
    \item Clique complex property: If $(U,V,W)$ is a triangle in $T(\{1\},\{2\},\{3\};\mu)$ then $\supp(\mu^{\{1,2,3\}})$ is non-empty.
\end{enumerate}
Then the tripartite graph $T(\{1,2\},\{3,4\},\{5,6\};\mu)$ has vanishing cohomology.
\end{lemma}

\begin{proof}
Let $\Phi$ be a fully triangle consistent instance on $G = \{(12,34,56),\mu\}$. We will show that there is a solution to the vertices that satisfies all the edges.

For each $i = 1$ and $V \in \supp(\mu|_{\{i\}})$, let $G(V)$ be the tripartite subgraph $T(\{2\},\{3,4\},\{5,6\};\mu|(X_1 = V))$ and same for $i=3,5$. Using the inductive hypothesis we can get a solution to the vertices of $G(V)$ that satisfies all the edges in $G(V)$. Let $L(V)$ be an ordered list of all such solutions. Note that the list is of size $m!$, since a fully-satisfiable solution to a  UG instance on a connected graph is unique upto symmetry of the permutations.

We will now create another UG instance $\Psi$ on the tripartite graph $H = T(\{1\},\{3\},\{5\};\mu)$ that is locally consistent. Consider an edge $(V,W)$ in this graph. First note that the subgraph $G(V) \cap G(W)$ must be non-empty and connected. Since there is a unique solution (upto symmetry) that satisfies the constraints in the intersection, the lists $L(V)$ and $L(W)$ must be equal when restricted to the vertices of $G(V) \cap G(W)$. So there exists a unique permutation $\pi_{V,W}$ such that for all $i \in [m!]$, $L(V)|_{G(V) \cap G(W)}[i] = L(W)|_{G(V) \cap G(W)}[\pi_{V,W}(i)]$.

Let us show that $\Psi$ is fully triangle consistent. Consider a triangle $(U,V,W)$ in $H$. Since $\mu$ has the clique complex property, the graph $G(U)\cap G(V)\cap G(W)$ is non-empty. We know that all the lists $L(U), L(V), L(W)$ assign the vertices in the intersection the same solution (since the satisfying solution is unique), therefore the permutations on the edges multiply to identity. We can now use the vanishing cohomology of $H$, since $\mu$ has local vanishing cohomology, to get a satisfying solution $S \in [m]^{V(H)}$ to $\Psi$. 

Let $L_i(V)$ denote the $i^{th}$ solution in the list $L(V)$ and let $L_i(V)[A]$ denote the permutation that  $L_i(V)$ assigns the vertex $A \in G$. For $A = (V_1,V_2) \in G$, assign it the permutation given by $L_{S(V_1)}[A]$ and similarly for vertices in the other two parts of $G$. We can now check that this solution satisfies all the constraints of $\Phi$. To do so, consider an edge $(A,B)=((V_1,V_2),(V_3,V_4))$. $(A,B)$ is satisfied by the solution $L_{S(V_1)}[A]$ and by the solution $L_{S(V_3)}[B]$. $(V_1,V_3)$ is an edge in $H$ and by construction, the lists $L(V_1),\pi_{V_1,V_3}(L(V_3))$ are consistent on their intersection, i.e. $L_{S(V_1)}[B] = L_{S(V_3)}[B]$. Therefore $(A,B)$ is satisfied by our assignment. This completes the proof that $G$ has vanishing cohomology.
\end{proof}

% When $i$ is odd and $\leq 2t-1$, $P_i(U,V)$ and $P_i(U,W)$ are in $P_2$ and they are of the form: $P_i(U,V) = (V_{(1)}, V_{(2)},\ldots, V_{(i/2)}, U_{(i/2+2)},\ldots, U_{(t)})$ and \\ ${P_i(U,V) = (V_{(1)}, V_{(2)},\ldots, V_{(\lfloor i/2\rfloor)}, U_{(\lfloor i/2\rfloor+2)},\ldots, U_{(t)})}$. We take the following path $R^i$ between them: 
% \begin{align*}
% R^i := &P_i(U,V) \rightarrow (W_{(1)},V_{(1)},\ldots, V_{(\lfloor i/2\rfloor)}, U_{(\lfloor i/2\rfloor+2)},\ldots, U_{(t)}) \\ 
% &\rightarrow (W'_{(1)},V_{(2)},\ldots, V_{(\lfloor i/2\rfloor)}, U_{(\lfloor i/2\rfloor+2)},\ldots, U_{(t)}) \rightarrow \ldots \rightarrow P_i(U,W),     
% \end{align*}
% that also alternates between vertices of dimension $k_2$ and $k_3$. 


% \begin{proof}
% Let $P_i(U,V)$ denote the subspace at the $i^{th}$-step of the path $P(U,V)$. We will give a triangulation $T(U,V,W)$ of the cycle with some repeating vertices, and ``equality'' edges between two vertices that are the same. Note that such a triangulation $T(U,V,W)$ yields a valid triangulation of the cycle (Definition~\ref{def:triangulation}) by identifying the repeating vertices, with the number of triangles involved being less than $|T(U,V,W)|$.

% This proof is broken into 3 cases depending on the dimensions of $V$ and $W$. We focus on the case that $(V,W)$ is an edge between $S_3$ and $S_2$. The analysis for the other two types of edges is exactly the same, hence we only discuss it briefly in the end. Let us assume that $W \in S_2$ and $V \in S_3$ with $W = (W_{(1)},\ldots,W_{(t-1)})$ and $V = (V_{(1)},\ldots, V_{(t)})$ being the block decomposition used in the paths from $U$ to $W$ and $V$. 

% \paragraph{Breaking $C(U,V,W)$ into smaller cycles $C^i$:}
% We first break $C(U,V,W)$ into $O(t)$ smaller cycles of length $O(t)$ each. We do so by creating paths $R^i(U,V,W)$ between $P_i(U,V)$ and $P_i(U,W)$ for even $i \leq 2t-2$, where $P_0(U,V) = P_0(U,W) = U$ and $P_1(U,V) = P_1(U,W) =(U_{(2)},\ldots,U_{(t)})$. For even $i \in [2,2t-2]$, $P_i(U,V)$ and $P_i(U,W)$ are in $S_3$ and are of the form $(V_{(1)},\ldots, V_{(i/2)}, U_{(i/2+1)},\ldots, U_{(t)})$ and $(W_{(1)},\ldots, W_{(i/2)}, U_{(i/2+1)},\ldots, U_{(t)})$ respectively. 


% We take the obvious path $R^i(U,V,W)$ between these vertices: 
% \begin{align*}
% R^i(U,V,W) := &P_i(U,V) \rightarrow (V_{(2)},\ldots, V_{(i/2)}, U_{(i/2+1)},\ldots, U_{(t)}) \\ &\rightarrow (W_{(1)},V_{(2)},\ldots, V_{(i/2)}, U_{(i/2+1)},\ldots, U_{(t)}) \rightarrow \ldots \rightarrow P_i(U,W),     
% \end{align*}
% that alternates between $k_3$ and $k_2$ dimensional vertices. Let us henceforth drop the notation $U,V,W$ in $R_i(U,V,W)$ since $U,V,W$ are fixed. Let $C^i(U,V,W)$ be the cycle $P_i(U,V) 
% \xrightarrow[]{R^{i}(U,V,W)} P_{i}(U,W) \rightarrow P_{i+1}(U,W) \rightarrow P_{i+2}(U,W) \xrightarrow[]{R^{i+2}(U,V,W)} P_{i+2}(U,V)\rightarrow P_{i+1}(U,V) \rightarrow P_{i}(U,V)$.

% \paragraph{Tiling $C^i$:} For notational simplicity, let us think of the cycle as: $(V_{(1)},\ldots, V_{(j)},U_{(j+1)},A) \rightarrow $


% As in the previous section, we first choose a random basis for vertices on the cycle.



% Let $P_i(U,V)$ be the first vertex on the path $R^i$, denoted by $R^i_1$ and let successive vertices on this path be denoted by $R^i_j$. Note that the paths $R^i$ and $R^{i+1}$ are of equal length when $i$ is even and furthermore $R^i_j$ and $R^{i+1}_j$ have an edge between them when $j$ is odd. This breaks the cycle $P_i(U,V) \rightarrow P_{i+1}(U,V) \rightarrow P_{i+1}(U,W) \rightarrow P_i(U,W) \rightarrow P_i(U,V)$ into multiple 6-cycles. When $i$ is odd, the path $R^{i+1}$ has length 2 more than $R^i$, but we still have that  $R^i_j$ and $R^{i+1}_j$ have an edge between them when $j$ is odd. As for the second to last vertex on $R^{i+1}$, it is the same as $P_i(U,W)$, the last vertex on $R^i(U,V,W)$ and therefore we have an equality edge between these, and the last vertex on $R^{i+1}$ is $P_{i+1}(U,W)$ which we know is connected to $P_i(U,W)$ too. This breaks the cycle $P_i(U,V) \rightarrow P_{i+1}(U,V) \rightarrow P_{i+1}(U,W) \rightarrow P_i(U,W) \rightarrow P_i(U,V)$ into 6-cycles and 2 triangles when $i$ is odd too. The only part of the cycle left to tile by 6-cycles/triangles is the cycle $P_{2t-1}(U,V) \xrightarrow[]{R^{2t-1}} P_{2t-1}(U,W) \rightarrow V \rightarrow P_{2t-1}(U,V)$. This cycle in fact breaks into triangles -- we claim that each vertex on $R^{2t-1}$ is connected to $V$, either by an edge in the graph or by an equality edge. It is definitely true for the first and last vertex, so let us consider the second vertex: $R^{2t-1}_2(U,V) = (W_{(1)}, V_{(1)},\ldots, V_{(t-1)})$. Since $W \subseteq V$, $W_{(1)} \in V$, therefore $R^{2t-1}_2(U,V) \subseteq V$. Since $\dim(R^{2t-1}_2(U,V)) = k_3$ (with high probability over the choice of the random bases for $V,W$), we get that $R^{2t-1}_2(U,V)= V$, therefore there is an equality edge between them. The same holds for all even vertices, and by the same argument every odd vertex is contained within $V$ too. 

% \paragraph{Tiling 8-cycles:}
% This shows that the whole cycle has been broken down into either triangles or 8-cycles. One can check that every 8-cycle created is isomorphic to the following 8-cycle: $(W_{(1)}, X) \rightarrow (W_{(1)}, W_{(2)}, X) \rightarrow (W_{(2)}, X) \rightarrow (V_{(1)}, W_{(2)}, X) \rightarrow (V_{(1)}, X) \rightarrow (W_{(1)}, V_{(1)}, X) \rightarrow (W_{(1)}, X)$, where $X$ is some $k_2 - (k_3-k_2) = 2k_2 - k_3$-dimensional subspace. Since $k_2-k_1 \geq k_3-k_2$, $\dim(X) \geq k_1$, which implies that there is some $k_1$-dimensional subspace $Y \subseteq X$ that is contained within all the vertices of the 6-cycle. Putting this vertex in the middle of the 6-cycle completes the triangulation of this 6-cycle, and similarly gives a triangulation of every 6-cycle in the decomposition of the original cycle. One can check that we used at most $O((k_3/k_3-k_2)^2)$-triangles in the triangulation, thus completing the proof of this case.

% \paragraph{$(V,W)$ is an edge between $P_3$ and $P_1$:}    
% Let $V = (V_{(1)},\ldots, V_{(t)})$ and $W = (W_{(1)},\ldots, W_{(t')})$ where $t'(k_3-k_2)=k_1$. Note that $P(U,W)$ has length $2t'+2$ whereas $P(U,V)$ has length $2t+1$. We first create the same paths $R^i$ between $P_i(U,V)$ and $P_i(U,W)$ when $i \leq 2t'$. Next we create paths between $P_i(U,V)$ and $P_{2t'+1}(U,W) = W$ which are again the ``obvious'' type of paths that we created above, i.e. they flip one block at a time and alternate between $k_3$ and $k_2$ dimensional subspaces, finally ending in the $k_1$-dimensional subspace $W$. One can again check that after putting in all the edges that exist between consecutive paths $R^i, R^{i+1}$, including the equality edges, the cycle breaks down into 6-cycles and triangles. These 6-cycles can be tiled in the same way as discussed above.

% \paragraph{$(V,W)$ is an edge between $P_2$ and $P_1$:} This follows the same proof as the above case hence we omit the details.   
% \end{proof}

% \textcolor{red}{The quotient attempt as we discussed doesn't quite achieve the simpler looking cycle. 
% The issue is that $(A,X_1)$ drops in dimension below the dimension of $A$. Probably best if we just to it straight.}
% Write $\F_q^{2d} = X+\wt{X}'$ where $\wt{X}' \cap X = \{0\}$.  Additionally let $\wt{X} = \wt{X}' \cap \symp(X)$, be the subspace of $\wt{X}'$ that is symplectically orthogonal to $X$; 
% note that $\dim(\wt{X})= 2d-2\dim(X)$. By shifting the subspaces, without loss of generality we can assume that all the subspaces $A,B,C,D$ are contained in $\wt{X}'$ and since they are contained in $\symp(X)$ we know that they are also contained withing $\wt{X}$. Henceforth we will therefore work in the ambient space $\wt{X}$, of dimension $2d' = 2d-2\dim(X)$. Let $k'_1=k_1-\dim(X')= k, k'_2=k_2-\dim(X)=2k$ and $k'_3 = k_3-\dim(X)$ that satisfies $d' \geq k'_3 \geq 3k$. We will show how to triangulate the cycle:
% \begin{align*}
% &(A,C) \rightarrow A \rightarrow (A,D) \rightarrow D \rightarrow (B,D) \\
% &\rightarrow B \rightarrow (B,C) \rightarrow C \rightarrow (A,C),
% \end{align*}
% with $k'_i$-dimensional subspaces also contained within $\wt{X}$. Adding back $X_1,X_2$ or $X$ appropriately to the vertices in the triangulation of the above cycle gives us a valid triangulation of the original cycle (since the vertices above intersect trivially with $X$).

%%%%%%%%%%%%%%%Third Induction using Global Hypercontractivity%%%%%%%%%%%

\subsection{An Inductive Bound on $C_{t,t,t}(\mu)$ via Global Hypercontractivity}
In this section, we present the
third and final inductive bound 
we need on $C_{t,t,t}(\mu)$.
The argument, once again, follows
similar lines, with one key difference. 
In contrast to previous arguments,
the subsets $S_1,S_2$ and $S_3$ 
we use will be of super constant
size $k$ (as opposed to just $3$ 
from previous arguments). This 
means that the number of iterations
we make is smaller by a factor 
of $1/k$, and therefore if we only
lose a constant factor in each 
iteration, the bound we get will
be substantially better than
the one in Lemma~\ref{lem:exp-bound-mu}. Towards this end, 
we need to use a corollary of 
global hypercontracitivity, 
which is Lemma~\ref{claim:event3} 
below.
\subsubsection{Auxiliary Claims}
We begin by setting up some machinery that is needed for the
argument in this section. 
In the following claim, we 
give upper bounds 
on the second largest singular
value of graphs that will arise
in our inductive argument.
\begin{claim}\label{claim:sing-val-H1}
Let $k \ll t \in \N$, $\mu$ be an $\eps$-product distribution over $\prod_{i \in [3]} \prod_{j \in R_i} X_j$ where $R_1,R_2,R_3$ are three $t$-sized disjoint sets of indices. Consider the collection $\cS$ of sets $S \subset_{3k} \cup R_i$ 
that satisfy $S \cap R_i = k, \forall i \in [3]$. Let $S_1,S_2$ be two disjoint sets in $\cS$ and let $(a_1,a_2) \in \mu^{S_1 \cup S_2}$ be some restriction of them. Consider the bipartite inclusion graph $H$ whose left side consists of the vertices $G_{a_1,a_2} = \cup_i \supp(\mu^{R_i}|(a_1,a_2))$, and its right side consists of pairs $(S,a)$, for $S \in \cS$ such that $S \cap (S_1 \cup S_2) = \emptyset$ and $a \in \supp(\mu^{S}|(a_1,a_2))$. An edge $(v, (S,a))$ in $H$ is sampled by picking a random $i\in [3]$, $v \sim \mu^{R_i}|(a_1,a_2)$, random $S \sim \cS$ conditioned on $(S \cap (S_1 \cup S_2) = \emptyset)$ and $a \sim \mu^S|(v,a_1,a_2)$. Then the second largest singular value of $H$ is $O(\sqrt{k^2/t})$.    
\end{claim}

\begin{proof}
Let $\cS'$ be the set of sets $S \in \cS$ with $S \cap (S_1 \cup S_2) = \emptyset$ and let $\cD$ be the distribution $\mu|(a_1,a_2)$. Let the left be called $L$ with the associated stationary distribution $\cD_L = \mu^{\cup R_i}|(a_1,a_2)$ and let the right side be called $R$ associated with the distribution $\cD_R$ over pairs $(S,a)$ where $S \sim \cS'$ and then $a \sim \mu^{S}|(a_1,a_2)$. Consider the operator $T:L_2(X_L;\cD_L) \rightarrow L_2(X_R;\cD_R)$ and the corresponding adjoint operator $T^{\dagger}: L_2(X_R;\cD_R) \rightarrow L_2(X_L;\cD_L)$. 

Let $g \in L_2(X_R;\cD_R)$ with $\E[g] = 0$ be the singular vector that achieves the second largest singular value of $M = TT^{\dagger}$. In the rest of the proof we will bound $\|Ag\|_2/\|g\|_2$. If it is $0$ we are done, so assume otherwise. We will use the following two facts in the proof:
\begin{enumerate}
\item  One can check that there exists a vector $f \in L_2(X_L;\cD_L)$ with $\E[f] = 0$ and $g = Tf$. Indeed, $g$ is an 
eigenvector of $M$ of eigenvalue 
$\lambda$, so 
$TT^{\dagger} g = \lambda g$, 
and we may take $f = \lambda^{-1}T^{\dagger} g$.
\item For $U,U' \in \cS'$, let $M'_{U',U}$ denote the submatrix of $M$ restricted to the rows $(U,a)$ for $a \in \supp(\cD^U)$ and columns $(U',a)$ for $a \in \supp(\cD^{U'})$ and let $M_{U',U} = |\cS'|M'_{U',U}$. We will now prove an upper bound on $\sigma_2(M_{U',U})$ when $U \cap U' = \emptyset$, where $\sigma_i(K)$ denotes the $i^{th}$-largest singular value of a matrix $K$. We have that $M_{U',U}:L_2(X_{U'};
\cD^{U'}) \rightarrow L_2(X_U;\cD^{U})$. One can check that $M_{U',U}$ can be written as:
\[M_{U',U} = \frac{1}{3}(M^{(1)}_{U',U}+M^{(2)}_{U',U}+M^{(3)}_{U',U}),\]
for $M^{(i)}_{U',U}f(x) = \E_{y \sim \cD|(X_{U \cap R_i} = x)}[f(y)]$. Furthermore, it holds that
\[
(M^{(i)}_{U',U})^\dagger M^{(i)}_{U',U} = (A_{U',U\cap R_i})^\dagger A_{U',U\cap R_i},
\]
where $A_{S,T}$ is the operator of the bipartite graph $A(S,T;\cD)$ from Definition~\ref{def:bip-mu}. Using Lemma~\ref{claim:gll-sing-val} to bound the singular value of $A_{U',U\cap R_i}$ we get that $\sigma_2(M^{(i)}_{U',U}) \leq \poly(r)\eps$. 
This implies that $\sigma_2(M_{U',U}) \leq \poly(r)\eps$.
\end{enumerate}

% For each $U\in \cS'$, let $g_U$ be the restriction of $g$ to ${\sf supp}(\cD^{U})$. For every vector $v \in L_2(X_R,\cD_R)$, let $v = [v_{U_1},\ldots, v_{U_m}]$ denote its decomposition into blocks corresponding to every $U_i \in \cS'$. 
% Consider the block decomposition of $g$:  $[g_{U_1},\ldots,g_{U_m}]$. 
Using the fact that $g = Tf$ for some $f$ with $\E[f]=0$, we get that for every $U \in \cS'$ we get, $\E_{a \sim \cD^{U}}[g_U(a)] = \E[Tf(a)] = \E[f] = 0$. Now, to bound $\|Mg\|_2^2$ we write it as $\E_{U \sim \cS'}[\|(Mg)_U\|_2^2]$ and upper bound it for each $U$ separately. For a fixed $U \in \cS'$ we have
\begin{align*}
\norm{(Mg)_U}_2 &= \norm{\sum_{U' \in \cS'}M'_{U',U}g_{U'}}_2 \\
&= \|\E_{U' \sim \cS'}[M_{U',U}g_{U'}]\|_2 \\
&\leq \E_{U' \sim \cS'}[\|M_{U',U}g_{U'}\|_2] ~~~~~~~\text{(by triangle inequality)}\\
&= \Pr_{U' \sim \cS'}[U' \cap U \neq \emptyset]\E_{\substack{U' \sim \cS'
\\ U'\cap U \neq \emptyset}}[\|M_{U',U}g_{U'}\|_2] + \Pr_{U' \sim \cS'}[U' \cap U=\emptyset]\E_{\substack{U' \sim \cS'
\\ U'\cap U = \emptyset}}[\|M_{U',U}g_{U'}\|_2] \\
&\lll \frac{k^2}{t}
\E_{\substack{U' \sim \cS'
\\ U'\cap U \neq \emptyset}}[\|g_{U'}\|_2] + \poly(r)\eps\E_{\substack{U' \sim \cS'\\ U'\cap U = \emptyset}}[\|g_{U'}\|_2].
\end{align*}
Squaring the above and using Cauchy-Schwarz we get that,
\[\|(Mg)_U\|_2^2 \lll \frac{k^4}{t^2}\E_{U' \sim \cS': U'\cap U \neq \emptyset}[\|g_{U'}\|^2_2] + \poly(r)\eps^2\E_{U' \sim \cS': U'\cap U = \emptyset}[\|g_{U'}\|^2_2].\]
Now to bound $\|Mg\|_2^2$, we can take an expectation over $U \sim \cS'$ for the above expression to get:
\begin{align*}
\|Mg\|_2^2 &\lll \E_{U \sim \cS'}\left[\frac{k^4}{t^2}\E_{U' \sim \cS': U'\cap U \neq \emptyset}[\|g_{U'}\|_2^2] + \eps^2\poly(r)\E_{U' \sim \cS': U'\cap U = \emptyset}[\|g_{U'}\|_2^2]\right]\\
&
\leq \frac{k^4}{t^2}\E_{U}[\|g_{U}\|_2^2] + \eps^2\poly(r) \E_{U}[\|g_{U}\|_2^2]\\
&\leq \frac{k^4}{t^2}\|g\|_2^2,
\end{align*}
which shows that $M$ has second largest eigenvalue $\leq O\left(\frac{k^2}{t}\right)$.
\end{proof}


\begin{claim}\label{claim:sing-val-H2}
Let $k \ll t \in \N$, $\mu$ be an $\eps$-product distribution over $\prod_{i \in [3]} \prod_{j \in R_i} X_j$ where $R_1,R_2,R_3$ are three $t$-sized disjoint sets of indices. Consider the set $\cS$ of sets $S \subset_{3k} \cup R_i$ 
that satisfy $S \cap R_i = k, \forall i \in [3]$ and let $S_1 \in \cS$, and $a_1 \in \mu^{S_1}$ be some restriction of $S_1$. Consider the bipartite inclusion graph $H$ whose left side consists of the vertices $G_{a_1} = \cup_{i \neq j \in [3]} \supp(\mu^{R_i\cup R_j}|a_1)$, and its right side consists of pairs $(S,a)$, for $S \in \cS$ such that $S \cap S_1 = \emptyset$ and $a \in \supp(\mu^{S}|a_1)$. An edge $(v, (S,a))$ in $H$ is sampled by picking a random $i\neq j\in [3]$, $v \sim \mu^{R_i\cup R_j}|a_1$, random $S \sim \cS$ conditioned on $S \cap S_1 = \emptyset$ and $a \sim \mu^S|(v,a_1)$. Then the second largest singular value of $H$ is $O(\sqrt{k^2/t})$.    
\end{claim}

\begin{proof}
We only sketch this proof since details are the same as Claim~\ref{claim:sing-val-H1}. Let $\cS'$ be the set of sets $S \in \cS$ with $S \cap S_1 = \emptyset$ and let $\cD$ be the distribution $\mu|a_1$. Let the left be called $L$ with the associated stationary distribution $\cD_L = \mu^{\cup R_i}|a_1$ and let the right side be called $R$ associated with the distribution $\cD_R$ over pairs $(S,a)$ where $S \sim \cS'$ and then $a \sim \mu^{S}|a_1$. Consider the operator $T:L_2(X_L;\cD_L) \rightarrow L_2(X_R;\cD_R)$ and the corresponding adjoint operator $T^{\dagger}: L_2(X_R;\cD_R) \rightarrow L_2(X_L;\cD_L)$. 

Let $g \in L_2(X_R;\cD_R)$ with $\E[g] = 0$ be the singular vector that achieves the second largest singular value of $M = TT^{\dagger}$. In the rest of the proof we will bound $\|Mg\|_2^2/\|g\|_2^2$. We will use the following two facts in the proof:
\begin{enumerate}
\item  One can check that there exists a vector $f \in L_2(X_L;\cD_L)$ with $\E[f] = 0$ and $g = Tf$. 
\item For $U,U' \in \cS'$, let $M'_{U',U}$ denote the submatrix of $M$ restricted to the rows $(U,a)$ for $a \in \supp(\cD^U)$ and columns $(U',a)$ for $a \in \supp(\mu^{U'}|(a_1,a_2))$ and let $M_{U',U} = |\cS'|M'_{U',U}$. We will now prove an upper bound on $\sigma_2(M_{U',U})$ when 
$U'$ and $U$ are disjoint. We have that $M_{U',U}:L_2(X_{U'};
\cD^{U'}) \rightarrow L_2(X_U;\cD^{U})$. One can check that $M_{U',U}$ can be written as:
\[M_{U',U} = \frac{1}{3}(M^{(1)}_{U',U}+M^{(2)}_{U',U}+M^{(3)}_{U',U}),\]
for $M^{(1)}_{U',U}f(x) = \E_{y \sim \cD|(X_{U \cap R_2 \cap R_3} = x)}[f(y)]$ and similarly for $M^{(2)}_{U',U}f(x),M^{(3)}_{U',U}f(x)$. Furthermore, we can check that $(M^{(i)}_{U',U})^\dagger M^{(i)}_{U',U} = (A_{U',U\cap R_j \cap R_k})^\dagger A_{U',U\cap R_j\cap R_k}$, for $j \neq k \neq i$ where $A_{S,T}$ is the operator of the bipartite graph $A(S,T;\cD)$ from Definition~\ref{def:bip-mu}. Using Lemma~\ref{claim:gll-sing-val} to bound the singular value of $A_{U',U\cap R_i}$ we get that $\sigma_2(M^{(i)}_{U',U}) \leq \poly(r)\eps$. 
This implies that $\sigma_2(M_{U',U}) \leq \poly(r)\eps$.
\end{enumerate}
The rest of the proof remains the same so we omit it.  \end{proof}

\subsubsection{A Corollary of Global Hypercontractivity}
The final ingedient we need it
an upper bound that the probability
a random restriction of a 
small subset of variables increases
the measure of a Boolean function
$f$ by a lot. Namely, suppose that 
$f\colon (\prod\limits_{i=1}^{d} X_i, \mu)\to\{0,1\}$ is a function, and we choose a random 
subset $S\subseteq_{k} [d]$ and 
restrict it randomly according 
to $x\sim \mu^{S}$. What 
is the probability that the 
measure of the restricted function, namely 
$\mu_{S\rightarrow x}(f)$, exceeds $\eta$ which is much larger than $\E[f]$? 
A naive application of Markov's
inequality shows this probability 
can be at most $\E[f]/\eta$; 
this bound is not good enough for
us however. Luckily, it turns
out that this bound is not tight
so long as $\eta$ is not too 
small, and the following improved 
bound can be proved:
\begin{lemma}\label{claim:event3}
There exists a constant $C>0$ 
such that the following holds.
Let $\cD$ be an $\eps$-product space over $X = \prod\limits_{i=1}^{d} X_i$, and let $f\colon X\to\{0,1\}$ be a function with $\E[f]\leq \frac{\eta}{100}$. If $\eps\leq 2^{-C\cdot \log(d)\log(1/\E[f])\log(1/\eta)}$, then for $k \leq d$,
\[
\Pr_{\substack{S \subset_k [d]\\ x\sim \cD^S}}\left[\mu_{S\rightarrow x}(f) \geq \eta\right]
\lll \frac{k}{d}\frac{\mu(f)}{\eta}\frac{\log(1/\eta)}{\log\log(1/\eta)}.
\]
\end{lemma}
\begin{proof}
Deferred to Section~\ref{sec:global-hyp}.
\end{proof}
% Let $\cD$ be an $\eps$-product measure over the domain $X_{1} \times \ldots \times X_m$ with $\eps \leq \exp(-m)$ and $f: \supp(\mu) \rightarrow \{0,1\}$ with $\mu(f) \in [\exp\left(-\sqrt{\frac{\log(1/\eps)}{\log m}}\right), \eta/100]$. Then,
% \[\Pr_{S \subset_k [m]}[\mu(f_{S \rightarrow a}) > \eta] \leq \frac{O(k)}{m}\mu(f)\sqrt{\log(1/\eta)}.\]

\subsubsection{The Inductive Argument}
We are now ready to give our 
third and final inductive 
bound on $C_{t}(\mu)$.
\begin{lemma}\label{lem:hard-recursion}
Let $k \ll t \leq r \ll d \in \N$ and $\mu$ over $\prod_{i \in I} X_i$ satisfy the assumptions in~\ref{assumption1}.
Assume that $\mu$ is a $(C_{t-k}(\mu),\beta_{t-k}(\mu))$-coboundary expander over $\S_m$. Let, 
\[B_t = C_{t-k}(\mu)\left(\frac{\exp(k\log(kr/t))}{t}\frac{\log(C_{t-k}(\mu))}{\log\log(C_{t-k}(\mu))}+ O(1)\right),\]
\[\beta_t = \beta_{t-k}\left(\frac{\exp(k\log(kr/t))}{t} + O(1)\right)+\exp(-r^{10})\exp(k\log(kr/t))\frac{\log(C_{t-k}(\mu))}{t\log\log(C_{t-k}(\mu))}.\]
Then $\mu$ is a $(C_t(\mu),\beta_t(\mu))$-coboundary expander over $\S_m$ with $C_t(\mu) \leq B_t$ and $\beta_t(\mu) \leq \beta_t$.
\end{lemma}

\begin{proof}
Fix any set $B \subseteq I$ of size at most $3r - 3t$, and $B_0 \in \supp(\mu^B)$, and let $R_1, R_2, R_3 \subset_{t} I \setminus B$ be disjoint sets. Let $\cD$ denote the distribution $\mu \mid X_B = B_0$ and let $\Phi$ be any UG instance on $G = T(R_1,R_2,R_3;\cD)$ with $\delta$-fraction of inconsistent triangles. It suffices to show that $\viol(\Phi) \leq B_t\delta+\alpha_t$. If $\delta \geq 1/B_t$, then this is immediately true, since $\viol(\Phi) \leq 1$. So henceforth let us assume that $\delta < 1/B_t$.

\paragraph{Setting up lists on restrictions:}
Consider the collection $\cS$ of sets $S \subset_{3k} \cup R_i$ 
that satisfy $S \cap R_i = k, \forall i \in [3]$. For every $S \in \cS$ and every restriction $a \in \supp(\mu^S)$, let $G_a$ be the subgraph $T(R_1,R_2,R_3;\cD|X_{S} = a)$. Let $X_a \in \S_m^{V(G_a)}$ be an assignment on $V(G_a)$ with maximum value, and let $L_{a}$ be an ordered list of solutions indexed by permutations in $\S_m$, where $L_{a}[\pi] = X_a\circ \pi$. 

\paragraph{Setting up permutations between restrictions:}
For every two disjoint sets $S_1, S_2 \in \cS$, and every restriction $a$ of $S_1$ and $b$ of $S_2$ where $(a,b) \in \supp(\cD^{S_1 \cup S_2})$, denote by $G_{a,b}$ the induced tripartite subgraph $T(R_1, R_2, R_3;\cD | (X_{S_1} = a,X_{S_2} = b))$. Let $\viol(X_a;G_{a,b})$ denote the fraction of edges in $G_{a,b}$ that are violated by the assignment $X_a$.
Then by Claim~\ref{claim:shift-partition} there exists a permutation $\pi_{a,b}$ that satisfies the following:
\begin{equation}\label{eq:bad-ij}
\Pr_{v \sim G_{a,b}}[X_a(v) \neq X_b(v)\pi_{a,b}] \leq \frac{\viol(X_a;G_{a,b})+\viol(X_b;G_{a,b})}{1-\lambda(G_{a,b})} \lll \viol(X_a;G_{a,b})+\viol(X_b;G_{a,b}),  
\end{equation}
where we used Claim~\ref{lem:eps-product-eigval} to bound $\lambda(G_{a,b})$ by $1/2+\poly(r)\eps \leq 0.51$. Let 
\[
\bad(a,b) = \{v\in G_{a,b}~|~X_a(v)\neq X_b(v)\pi_{a,b}\}.
\]
For any restriction $b$ as above, let $L_b\circ \pi$ denote the list where $L_b\circ \pi[\pi'] = L_b[\pi\pi'] = X_b\circ\pi\pi'$. With these notations and the definition of $\bad(a,b)$, we get that $L_a|_{G_{a,b} \cap \overline{\bad(a,b)}} = L_b\circ\pi_{a,b}|_{G_{a,b} \cap \overline{\bad(a,b)}}$. 

\paragraph{Counting bad triangles:}
Consider any three disjoint sets $S_1,S_2,S_3 \in \cS$ and any restrictions $a_1,a_2,a_3$ of $S_1,S_2,S_3$ respectively where $(a_1,a_2,a_3) \in \supp(\cD^{\cup S_i})$. Let $G_{S_1\rightarrow a_1,S_2\rightarrow a_2, S_3\rightarrow a_3}$ denote the graph $T(R_1, R_2, R_3;\cD|(a_1,a_2,a_3))$. We say a tuple $(a_1,a_2,a_3)$ is bad if either of the following holds:
\begin{enumerate}
\item $\mu_{G_{a_1,a_2,a_3}}(\bad(a_i,a_j)) > 1/100 + \mu_{G_{a_1,a_2}}(\bad(a_1,a_2))$ for some $i \neq j \in [3]$.
\item $\viol(X_{a_i}; G_{a_i,a_j}) > 1/100 + \viol(X_{a_i})$ for some $i \neq j \in [3]$.
\item $\viol(X_{a_i}) > 1/100$ for some $i \in [3]$.
\end{enumerate}

Let us now bound the probability that each of these events happens over a random choice of $S_i$'s and $a_i$'s, starting with event (1). Fix $a_1, a_2$ and vary $a_3$. Clearly, we have that
\[\E_{\substack{S_3 \sim \cS|S_3 \cap (S_1 \cup S_2)=\phi\\a_3 \sim \cD^{S_3}|(a_1,a_2)}}[\mu_{G_{a_1,a_2,a_3}}(\bad(a_1,a_2))] = \mu_{G_{a_1,a_2}}(\bad(a_1,a_2)).\]
Consider the bipartite inclusion graph $H_1$ whose left side consists of the vertices of $G_{a_1,a_2}$, and its right side consists of possible restrictions $a_3$ (where $S_3 \in \cS$ varies). By Claim~\ref{claim:sing-val-H1} the largest singular value of $H_1$ is at most $O(\sqrt{k^2/t})$, therefore by Lemma~\ref{lem:sampling} and~\eqref{eq:bad-ij} we get:
\begin{align*}
&\Pr_{\substack{S_3\sim \cS|S_3 \cap (S_1\cup S_2) =\emptyset \\ a_3 \sim \cD^{S_3}|(a_1,a_2)}}\left[\mu_{G_{a_1,a_2,a_3}}(\bad(a_1,a_2)) > \frac{1}{100}+\mu_{G_{a_1,a_2}}(\bad(a_1,a_2))\right]\\
&\qquad\qquad\lll \frac{k^2}{t}(\viol(X_{a_1};G_{a_1,a_2})+\viol(X_{a_2};G_{a_1,a_2})), \end{align*}
which then implies that,
\begin{align}
&\Pr_{\substack{S_1,S_2,S_3\sim \cS:S_i\cap S_j = \emptyset~\forall i\neq j\\ (a_1,a_2)\sim\mathcal{D}^{S_1\cup S_2} \\ a_3 \sim \cD^{S_3}|(a_1,a_2)}}[\mu_{G_{a_1,a_2,a_3}}(\bad(a_1,a_2)) > \frac{1}{100}+\mu_{G_{a_1,a_2}}(\bad(a_1,a_2))]\nonumber\\
&\qquad\qquad\lll \frac{k^2}{t}\E_{\substack{S \sim \cS\\ a \sim \cD^S}}[\viol(X_{a})] \notag\\
&\qquad\qquad\lll \frac{k^2}{t}(C_{t-k}\delta+\beta_{t-k}),\label{eq:bad1}
\end{align}
where we applied the coboundary guarantee on the graphs $G_a$.


Let us now bound the probability of the bad event (2). As above, first fix an $S_1, a_1$ and then vary $S_2, a_2$. Let $H_2$ be the weighted bipartite inclusion graph with the left side consisting of the edges in $G_{a_1}$ and the right side consisting of $(S_2, a_2)$ (the weights determined using $\mu$). Similar to the above argument, we can use the largest singular value of $H_2$ (Claim~\ref{claim:sing-val-H2}) to get that
\[
\Pr_{\substack{S_2\sim \cS:S_2 \cap S_1 =\phi \\ a_2 \sim \cD^{S_2}|a_1}}[\viol(X_{a_1};G_{a_1,a_2}) > \frac{1}{100}+\viol(X_{a_1})]
\lll \frac{k^2}{t}\viol(X_{a_1}),
\]
an taking expectation over 
$a_1$ gives that
\[
\Pr_{\substack{S_2\sim \cS:S_2 \cap S_1 =\emptyset\\ a_1\sim \mathcal{D}^{S_1}\\ a_2 \sim \cD^{S_2}|a_1}}[\viol(X_{a_1};G_{a_1,a_2}) > \frac{1}{100}+\viol(X_{a_1})]
\lll \frac{k^2}{t}\E_{\substack{S \sim \cS\\ a \sim \cD^S}}[\viol(X_{a})] \lll\frac{k^2}{t}(C_{t-k}\delta+\beta_{t-k}).
\]

%Therefore we have that $\alpha < 1/B_t$ and $\eps < \exp(-r\log r\log(1/\alpha))$ for all $t \leq r$. 

To bound event (3), we use Lemma~\ref{claim:event3} on $f: \prod_{i\in R_1\cup R_2\cup R_3} X_i \rightarrow \{0,1\}$ defined as $f(a_1,a_2,a_3) = \Ind((a_1,a_2,a_3) \in \incons(\Phi))$. Let us now verify that the hypotheses of the lemma are satisfied. Set $\alpha = \exp(-r^{10})$. We have that $\E[f] = \delta$, which might be too small, therefore after turning some values of $f$ from $0$ to $1$ we can safely assume that $\E[f] =\max(\delta,\alpha)$. We will bound the probability that $\delta_a > \eta: = \frac{1}{100C_{t-k}}$, where $\delta_a$ is the fraction of violated triangles seen inside $G_a$. Since $\E[f] \geq \alpha$ and $\eta = \frac{1}{100C_{t-k}}$, for $C_{t-k} \leq 2^{O(r\log r)}$ by Lemma~\ref{lem:exp-bound-mu} and $\eps = \exp(-r^{12})$ we have that 
\[
\eps < \exp(-C\log r\log(1/\E[f])\log(1/\eta))
\]
for sufficiently large constant $C$. We can use Lemma~\ref{lem:exp-bound-mu} to conclude that $B_t \leq \exp(r\log r)$ which implies that $\alpha < 1/B_t$. This gives us that $\E[f] < \eta/100$, because if this wasn't the case then, 
\[
\frac{\eta}{100}
=
\frac{1}{100^2 C_{t-k}} 
\leq \E[f]
\leq 
\delta+\alpha < \frac{1}{B_t}+\alpha \leq \frac{2}{B_t},
\] and rearranging we get that $B_t < 20000 C_{t-k}$, which is a contradiction to the choice of $B_t$ when we take 
the implicit constant $O(1)$ 
there to be at least $20000$. This shows that both the hypothesis of Lemma~\ref{claim:event3} are satisfied, hence applying the lemma on $f$ we get,
\[
\Pr_{\substack{S \sim \cS\\a \sim \cD^S}}
\left[\delta_a > \frac{1}{100C_{t-k}}
\right] \leq \frac{\poly(k)}{t}\frac{\log(C_{t-k})}{\log\log(C_{t-k})}C_{t-k}(\delta+\alpha).\]  
Technically, a direct application of the lemma would have $S \subset_{3k} \cup R_i$, whereas above we have $S \sim \cS$. But since the probability that $|S \cap R_i| = k, \forall i$ is at least $1/\poly(k)$ the above statement readily follows.

Taking a union bound over these events we get,
\begin{equation}\label{eq1}
\Pr_{\substack{S_1,S_2,S_3 \sim \cS: S_i\cap S_j =\emptyset~\forall i\neq j\\(a_1,a_2,a_3) \sim \cD^{\cup S_i}}}[(a_1,a_2,a_3) \text{ is bad}]
\lll \frac{\poly(k)}{t}\frac{\log(C_{t-k})}{\log\log(C_{t-k})}C_{t-k}(\delta+\alpha)+ \frac{k^2}{t}\beta_{t-k}.
\end{equation}
Let $r' = r\log\log\log r$. To obtain the condition that $\cup S_i$ is $\Omega(td/kr')$-separated we can use Claim~\ref{claim:random-separated} to get that:
\[\Pr_{\substack{S_1,S_2,S_3 \sim \cS:\cap S_i = \emptyset}}\left[\min_{a \neq b \in \cup S_i}|a-b| \geq \Omega\left(\frac{td}{kr'}\right)\right] \geq 
2^{-O(k)},\]
where we used the fact that $(\cup S_i) \cap R_1$ is distributed as a uniform set $U_1 \subset_k R_1$ and the same holds for the intersection with $R_2$ and $R_3$. Let $\cS'$ be the set of $(S_1,S_2,S_3)$ satisfying $S_i \in \cS$, $S_i\cap S_j = \emptyset$ for $i\neq j$ and $\cup S_i$ is $\Omega(td/kr')$-separated. Then using \eqref{eq1} we get that,
\begin{equation*}%\label{eq2}
\Pr_{\substack{S_1,S_2,S_3 \sim \cS:\cap S_i =\emptyset\\(a_1,a_2,a_3) \sim \cD^{\cup S_i}}}[(a_1,a_2,a_3) \text{ is bad}\mid (S_1,S_2,S_3) \in \cS']
\leq \frac{\exp(k)}{t}\frac{\log(C_{t-k})}{\log\log(C_{t-k})}C_{t-k}(\delta+\alpha)+\frac{\exp(k)}{t}\beta_{t-k},
\end{equation*}
and we denote the right hand side by $\delta''$. Therefore there exist disjoint sets $S_1,S_2,S_3$ where $\cup S_i$ is well-separated and where the graph $T(S_1,S_2,S_3;\cD)$ has at most $\delta''$-fraction of bad triangles (as defined above). We fix such $S_1,S_2,S_3$ henceforth.

\paragraph{Creating a UG instance on graph over restrictions:}
Let $\Psi$ be the following UG instance on $H = T(S_1,S_2,S_3;\mu)$: each edge $(a_i,a_j)$ has the constraint $\pi_{a_i,a_j}^{-1}$. That is, we want to find a solution $A$ that maximizes the fraction of edges satisfying $A(a_i) = \pi_{a_i,a_j}^{-1}A(a_j)$. Note that a triangle $(a_1,a_2,a_3)$ is consistent if $\pi_{a_3,a_1}^{-1}\pi_{a_1,a_2}^{-1}\pi_{a_2,a_3}^{-1} = \text{id}$ or equivalently if $\pi_{a_2,a_3}\pi_{a_1,a_2}\pi_{a_3,a_1} = \text{id}$.

First note that if a triangle $(a_1,a_2,a_3)$ is not bad, then it is consistent. This is because when all the events hold, for all $i \neq j$ we get:
\begin{align*}
\mu_{G_{a_1,a_2,a_3}}(\bad(a_i,a_j)) &\leq \frac{1}{100} +\mu_{G_{a_i,a_j}}(\bad(a_i,a_j))\\ 
&\leq \frac{1}{100}+2(\viol(X_{a_i};G_{a_i,a_j})+\viol(X_{a_j};G_{a_i,a_j}))\\
&\leq \frac{1}{100}+ \frac{6}{100}+ 3(\viol(X_{a_i})+\viol(X_{a_j})) \\
&\leq \frac{13}{100}. 
\end{align*}
This says that $\mu_{G_{a_1,a_2,a_3}}(\bad(a_1,a_2) \cup \bad(a_2,a_3) \cup \bad(a_1,a_3)) \leq 3\cdot (13/100)$, which gives that 
$\mu_{G_{a_1,a_2,a_3}}(\good(a_1,a_2,a_3)) \geq 0.5 > 0$, where the latter set is defined as those vertices in $G_{a_1,a_2,a_3}$ that don't belong to any of $\bad(a_i,a_j)$. We have that: 
\begin{align*}
L_{a_1}|_{\good(a_1,a_2,a_3)} = L_{a_2}\circ \pi_{a_1,a_2}|_{\good(a_1,a_2,a_3)}\\
L_{a_2}|_{\good(a_1,a_2,a_3)} = L_{a_3}\circ \pi_{a_2,a_3}|_{\good(a_1,a_2,a_3)}\\
L_{a_3}|_{\good(a_1,a_2,a_3)} = L_{a_1}\circ \pi_{a_3,a_1}|_{\good(a_1,a_2,a_3)},
\end{align*}
which implies that: 
\[L_{a_3}|_{\good(a_1,a_2,a_3)} = L_{a_3}\circ \pi_{a_2,a_3}\circ \pi_{a_1,a_2}\circ \pi_{a_3,a_1}|_{\good(a_1,a_2,a_3)} = L_{a_3}\circ\pi_{a_2,a_3}\pi_{a_1,a_2}\pi_{a_3,a_1}|_{\good(a_1,a_2,a_3)}.\] 
Taking any $v \in {\good(a_1,a_2,a_3)}$ we get that, $L_{a_3}[\text{id}][v] = L_{a_3}\circ \pi_{a_2,a_3}\pi_{a_1,a_2}\pi_{a_3,a_1}[\text{id}][v]$, where the former is $X_{a_3}(v)$ and the latter is $X_{a_3}(v)\pi_{a_2,a_3}\pi_{a_1,a_2}\pi_{a_3,a_1}$, which implies $\pi_{a_2,a_3}\pi_{a_1,a_2}\pi_{a_3,a_1} = \text{id}$. 

Using the coboundary expansion of the graph $T(S_1,S_2,S_3;\cD^{\cup S_i})$, we get that there exists a UG solution $A$ to the vertices violating at most $C(T(S_1,S_2,S_3;\cD^{\cup S_i}))\delta''$-fraction of the edges. Since $\cup S_i$ is $\Omega(td/kr')$-separated, $C_{1}(\cD^{\cup S_i}) \leq \poly(kr'/t)$ and using Lemma~\ref{lem:easy-recursion} we get that 
\[
C_{3k}(\cD^{\cup S_i}) \leq \poly(kr'/t)^{k} = \exp(k \log(kr'/t)).
\]
Therefore $\viol(A) \leq \exp(k \log(kr'/t))\delta'':=\delta'$. 

\paragraph{Lifting the solution:} We can now use $A$ to create a good solution $B$ to $G = T(R_1,R_2,R_3;\cD)$. The proof is identical to Lemma~\ref{lem:exp-bound-mu} hence we omit it here. We get that there exists an assignment $B$ that violates at most $O(\delta' + C_{t-k}\delta+\beta_{t-k}) = B_t \delta+\beta_t$-fraction of the edges of $G$, which completes the proof.
\end{proof}
% We will now use $A$ to create a highly satisfying solution $B$ to $G = T(R_1,R_2,R_3;\mu)$. For every vertex $v \in R_i$ and restriction $a \in \supp(\mu^{S_1}|(X_{R_i} = v))$, let $g_a(v)$ denote the permutation $L_{a}[A(a)][v]$. We will choose a randomized assignment as follows: to every vertex $u \in R_i$, choose a random $s \sim \cD^{S_1}|(X_{R_i} = u)$ and assign $B(u)= g_{s}(u)$. We will now upper bound the expected fraction of edges that $B$ violates for $\Phi$. 

% Consider an edge $(u_i,u_j) \in G$ between parts $R_i,R_j$. This edge is satisfied if there exists $s \in \supp(\cD^{S_1}|(X_{R_i} = u_i, X_{R_j} = u_j))$ such that, (1) $B(u_i) = g_s(u_i)$, (2) $B(u_j) = g_s(u_j)$ and (3) The assignment $(g_s(u_i),g_s(u_j))$ satisfies the edge $(u_i,u_j)$ or equivalently $(u_i,u_j)$ is satisfied by the assignment $X_s$. So let us calculate the probability that each event does not hold, starting with event (1).
% \begin{align*}
% &\E_B\E_{(u_i,u_j) \sim G}\E_{s \sim \cD^{S_1}|(X_{u_i} = R_i, X_{u_j} = R_j)}[\Ind(B(u_i) \neq g_s(u_i))]\\
% =&\E_{u \in G}\E_{s,s' \sim \cD^{S_1}|u}[\Ind(g_{s'}(u) \neq g_s(u))]. 
% \end{align*}

% To calculate this, let us first calculate a bound on:
% \[\E_{u \in G}\E_{\substack{i\neq j \in [3]\\(s,s') \sim \cD^{S_i \cup S_j}|u}}[\Ind(g_{s'}(u_i) \neq g_s(u_i))].\]
% Fix a vertex $u \in R_i$ for some $i$. It is easy to check that an edge $(s,s') \in T(S_1,S_2,S_3;\cD|u)$ satisfies $g_s(u) = g_{s'}(u)$ if $(s,s') \notin \viol(A)$ and $u \notin \bad(s,s')$. Therefore,
% \begin{align*}
% &\E_{u \in G}\E_{\substack{i\neq j \in [3]\\(s,s') \sim \mu^{S_i \cup S_j}|u}}[\Ind(g_{s'}(u) \neq g_s(u))]\\
% &\leq \E_{u \in G}\E_{\substack{i\neq j \in [3]\\(s,s') \sim \cD^{S_i \cup S_j}|u}}[\Ind((s,s') \in \viol(A))]+\E_{u \in G}\E_{\substack{i\neq j \in [3]\\(s,s') \sim \cD^{S_i \cup S_j}|u}}[\Ind(u \in \bad(s,s'))]\\
% &= \viol(A) + \E_{\substack{(s,s') \sim E(T(S_1,S_2,S_3;\cD))\\ u \in G_{s,s'}}}[\Ind(u \in \Bad(s,s'))]\\
% &=\delta' + 2\E_{s \in T(S_1,S_2,S_3;\cD)}[\viol(X_u)]\\
% &\leq \delta'+ O(C_{t-k})\delta+O(\beta_{t-k}).
% \end{align*}

% We are ready to bound the probability that event (1) does not happen. Let $p_u := \Pr_{\substack{(s,s') \sim \cD^{S_1 \cup S_2}|u}}[g_{s'}(u) \neq g_s(u)]$. By the above we know that $\E_{u \in G}[p_u] \leq O(\delta' + C_{t-k}\delta)$. Let $p'_u = \Pr_{\substack{s,s' \sim \cD^{S_1}|u}}[g_{s'}(u) \neq g_s(u)]$. Using the fact that the second largest singular value of the bipartite graph $B(S_1,S_2;\cD|u)$ is $\ll 1/2$ for all $u$ (Lemma~\ref{claim:gll-sing-val}) we get that, $p'_u \leq O(p_u)$, which gives us that,
% \[\E_{u \in G}\E_{s,s' \sim \cD^{S_1}|u}[\Ind(g_{s'}(u) \neq g_s(u))] \leq O(\delta'+ C_{t-k}\delta+\beta_{t-k}),\]
% thus bounding the probability of event (1). One can check that the probability of event (2) is the same as event (1), hence let us proceed to event (3). For that we get,
% \[\E_{(u_i,u_j) \sim G}\E_{s \sim \cD^{S_1}|(X_{u_i} = R_i, X_{u_j} = R_j)}[\Ind((u_i,u_j) \in \viol(X_s))] \leq C_{t-k}\delta+\beta_{t-k}.\]



\begin{lemma}\label{lem:main-local-to-global}
Let $r,d \in \N$, $r \ll d$, and let $\mu$ over $\prod_{i \in I} X_{i}$ satisfy the assumptions \ref{assumption1}. Then $\mu$ is a $(C_r,\beta_r)$-coboundary expander over $\S_m$ with $C_r \leq \exp(r\log\log\log r/\log\log r)$ and $\beta_r \leq 2^{-\Omega(r^{10})}$.    
\end{lemma}

% Let $k,t,r,d \in \N$ with $t \in [r/\log^3r,r]$, $k \ll t \leq r \ll d$ and $\eps,\alpha \in (0,1)$ and let $I = \{i_1,\ldots,i_{3r}\} \subseteq_{3r} [d]$ with $\min_{a\neq b \in [3r]}(|i_a - i_b|) \geq \Omega(d/r)$. Let $\mu$ be an $\eps$-product distribution over $\prod_{i \in I} X_i$, that is also a $(C_{t-k}(\mu),\beta_{t-k}(\mu))$-coboundary expander over $\S_m$ with $C_{t-k}(\mu) \leq \exp(r\log r)$ and let $\eps \leq \exp(-r\log r\log(1/\alpha))$. Let $\cT$ be the set of all triples $(S_1,S_2,S_3)$ with $S_i \subset_k I$ being pairwise disjoint and $\min_{a\neq b \in \cup_i S_i}(|i_a - i_b|) \geq \Omega(td/kr)$, and let $K = \max_{(S_1,S_2,S_3) \in \cT}(C(T(S_1,S_2,S_3);\mu))$. Let, 
% \[B_t = C_{t-k}(\mu)\left(\frac{\exp(k)}{t}\frac{\log(C_{t-k}(\mu))}{\log\log(C_{t-k}(\mu))}K+ O(1)\right),\]
% \[\beta_t = \beta_{t-k}\left(\frac{\exp(k)}{t}K + O(1)\right)+\alpha K\frac{\exp(k)\log(C_{t-k}(\mu))}{t\log\log(C_{t-k}(\mu))}.\]
% and $\alpha < 1/B_t$. Then $\mu$ is a $(C_t(\mu),\beta_t(\mu))$-coboundary expander with $C_t(\mu) \leq B_t$ and $\beta_t(\mu) \leq \alpha_t$.


\begin{proof}
Set $t_0 = \Theta(r/\log\log r), r' = r\log\log\log r$ and $k = \Theta(\log\log r/\log\log\log r)$. We can now apply Lemma~\ref{lem:hard-recursion} with these parameters to get that for all $\ell \in [0,(r-t_0)/k]$:
\begin{equation}\label{eq:recursion-hard}
C_{t_0+(\ell+1)k}(\mu) \leq  C_{t_0+\ell k}(\mu)\left(\frac{\exp(k\log(kr'/t))}{t_0+\ell k}\frac{\log(C_{t_0+\ell k}(\mu))}{\log\log(C_{t_0+\ell k}(\mu))}+ O(1)\right).
\end{equation}
We will show that for all $\ell \in [0,(r-t_0)/k]$: 
\begin{equation}\label{eq:recursion1}
C_{t_0+\ell k} \leq \exp(t_0\log(r'/t_0))\cdot \exp(\ell).    
\end{equation}
Let us prove this by induction on $\ell$. By Lemma~\ref{lem:exp-bound-mu} we know that $C_{t_0}(\mu) \leq \exp(t_0\log(r'/t_0))$, hence the above holds for $\ell = 0$. Assume the hypothesis for $\ell$ and let us prove it for $\ell+1$. Applying \eqref{eq:recursion-hard} we get that,
\begin{align*}
C_{t_0+(\ell+1)k}(\mu) &\leq  C_{t_0+\ell k}(\mu)\left(\frac{\exp(k\log(kr'/t))}{t_0+\ell k}\frac{\log(C_{t_0+\ell k}(\mu))}{\log\log(C_{t_0+\ell k}(\mu))}+ O(1)\right)\\
&\leq \exp(t_0\log(r'/t_0))\cdot \exp(\ell) \cdot O(1)\\
&\leq \exp(t_0\log(r'/t_0))\cdot \exp(\ell+1),
\end{align*}
where we used the fact that $\frac{\exp(k\log(kr'/t))}{t}\frac{\log(C_{t_0+\ell k}(\mu))}{\log\log(C_{t_0+\ell k}(\mu))} = o(1)$. This proves \eqref{eq:recursion1}, thus showing that $C_r \leq \exp(r\log\log\log r/\log\log r)$.
As for bounding $\beta_t$ we can use the fact that $\beta_{t_0} = \exp(-r^{12})$ (Lemma~\ref{lem:exp-bound-mu}) and then use induction to show that $\beta_t \leq \exp(t)\beta_{t_0} \leq 2^{-\Omega(r^{10})}$.
\end{proof}





